Physical Design Obfuscation of Hardware: A Comprehensive Investigation of Device- and Logic-Level Techniques

The threat of hardware reverse engineering is a growing concern for a large number of applications. A main defense strategy against reverse engineering is hardware obfuscation. In this paper, we investigate physical obfuscation techniques, which perform alterations of circuit elements that are difficult or impossible for an adversary to observe. The examples of such stealthy manipulations are changes in the doping concentrations or dielectric manipulations. An attacker will, thus, extract a netlist, which does not correspond to the logic function of the device-under-attack. This approach of camouflaging has garnered recent attention in the literature. In this paper, we expound on this promising direction to conduct a systematic end-to-end study of the VLSI design process to find multiple ways to obfuscate a circuit for hardware security. This paper makes three major contributions. First, we provide a categorization of the available physical obfuscation techniques as it pertains to various design stages. There is a large and multidimensional design space for introducing obfuscated elements and mechanisms, and the proposed taxonomy is helpful for a systematic treatment. Second, we provide a review of the methods that have been proposed or in use. Third, we present recent and new device and logic-level techniques for design obfuscation. For each technique considered, we discuss feasibility of the approach and assess likelihood of its detection. Then we turn our focus to open research questions, and conclude with suggestions for future research directions.

==> open-research.tex <==
open research questions go here

==> structural.tex <==
\deh{we wanted to have something about structural information, but I am not sure if it should be its own section}

Circuit structure information can also leak significant information about a design. For example, flip flops and latches can easily be identified by following clock signals. SRAM is apparent by its structure, and in order to obfuscate SRAM it would need to be implemented as a register file. 

Hierarchy in chip integration reveals information. Hard IP is typically confined to lower metal layers, and signals in upper metal layers can be identified as inter-block signals. Buses or on-chip networks should be relatively easy to identify as wide collections of wires running together between a common set of agents.

As the predictable on-chip structures are designed for efficiency, any attempt to conceal structural information will pay a cost in performance, area, or integration complexity.


